Feedback-Aware Precoding for Millimeter Wave Massive MIMO Systems

Millimeter wave (mmWave) communication is a promising solution for coping with the ever-increasing mobile data traffic because of its large bandwidth. To enable a sufficient link margin, a large antenna array employing directional beamforming, which is enabled by the availability of channel state information at the transmitter (CSIT), is required. However, CSIT acquisition for mmWave channels introduces a huge feedback overhead due to the typically large number of transmit and receive antennas. Leveraging properties of mmWave channels, this paper proposes a precoding strategy which enables a flexible adjustment of the feedback overhead. In particular, the optimal unconstrained precoder is approximated by selecting a variable number of elements from a basis that is constructed as a function of the transmitter array response, where the number of selected basis elements can be chosen according to the feedback constraint. Simulation results show that the proposed precoding scheme can provide a near-optimal solution if a higher feedback overhead can be afforded. For a low overhead, it can still provide a good approximation of the optimal precoder.

==> sections/Feedback.tex <==
\section{Feedback-Aware Precoder Design}\label{sec:feedback}

In this section, we design an adaptive precoder for \gls{mmWave} massive \gls{MIMO} systems. We first discuss the proposed design methodology and then analyze the corresponding feedback overhead. % and the complexity.

\subsection{Proposed Precoder Design}\label{subsec:precoder}
We start by examining the structure of the optimal unconstrained precoder. In particular, given the singular-value decomposition of the channel $\mat H=\mathbf{U}\boldsymbol{\Sigma}\mathbf{V}\hermis$, the optimal linear precoder that maximizes the mutual information between $s$ and $y$ is $\Fopt= [\alpha_1\mathbf{v}_1,\dots,\alpha_s\mathbf{v}_S]$, where column vector $\mat{v}_s\in \set C^{M\times1}$ is the right singular vector corresponding to the $s$-th largest singular value and $\alpha_s$ is the power allocation factor for the $s$-th stream and has to satisfy $\frac{1}{S}\sum_s \alpha_s^2=1$ and can be obtained with the water-filling algorithm~\cite{biglieri2007mimo}.
Additionally, given the clustered channel model in \eqref{Eq:Channel}, we can give a compact representation \mbox{$\mat H = \mat H_r \bar{\mat H} \mat H_t\hermis$},
where $\mat H_r = \big[\mathbf{h}_r(\theta_{1}),\dots,\mathbf{h}_r(\theta_{LJ})\big]\in \set C^{N\times LJ}$ and
\mbox{$\mat H_t=\big[\mathbf{h}_t(\phi_{1}),\dots,\mathbf{h}_t(\phi_{LJ})\big] \in \set C^{M\times LJ}$} are the receiver and transmitter array response matrices at specific \glspl{AoA} and \glspl{AoD}, respectively, and $\bar{\mat H}$ is a diagonal matrix containing the coefficients of all rays/path in all clusters. Given the previous observations, it can be shown that the optimal precoder can be written as $\Fopt=\sum_{k=1}^{LJ} \mat h_t(\phi_k)\mat{g}_k\hermis$, where $\phi_k$ is the $k$-th channel \gls{AoD} and $\mat{g}_k\in\set C^{S\times 1}$ is the corresponding appropriate combining vector \cite{el2014spatially}.

Based on the above, we propose to approximate the optimal precoder as follows
%%%%%%%%%%%%%%%%%% Equation %%%%%%%%%%%%%%%%%% 
\begin{IEEEeqnarray}{lll} \label{Eq:precoder}
(\phiopt, \Gopt)= \underset{\boldsymbol{\phi} \in \Cphi^{K\times 1}, \mat{G}\in\set C^{K\times S}}{\mathrm{argmin}} \frob{\Fopt-\CHt(\boldsymbol{\phi}) \mat{G}},
\end{IEEEeqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%where $\Cphi$ is channel \glspl{AoD} codebook as
%\begin{IEEEeqnarray}{lll} \label{Eq:cphi}
%\Cphi = \Big\{\phi_\mathrm{min}+{\phi_\mathrm{sector} \over 2|\Cphi|},\phi_\mathrm{min}+{3\phi_\mathrm{sector} \over 2|\Cphi|},\cdots, \phi_\mathrm{max}-{\phi_\mathrm{sector} \over 2|\Cphi|}\Big\},	
%\end{IEEEeqnarray}
%
%where $\CHt(\Cphi)$ is naturally defined as the transmitter array response matrix at all angles in the channel \glspl{AoD} codebook $\Cphi$, which is written as
%\begin{IEEEeqnarray}{lll} \label{Eq:CHt}
% \CHt(\Cphi)=\big[\mathbf{h}_t(\phi_1),\cdots,\mathbf{h}_t(\phi_{|\Cphi|})\big], 
%\end{IEEEeqnarray}
%and discussed in more detail in Section~\ref{subsec:non-modulo-one},
%$\phiopt$ is the set of best $\K$ angles from $\Cphi$,
%$\Gopt=[\mat{g}_1,\cdots,\mat{g}_\K]\hermis$ is the appropriate combining matrix,
%and $\K$ is a design parameter that can be chosen according to the feedback link bandwidth constraints.
%
where $\mat{G}\in\set C^{K\times S}$ is the combining matrix and $\CHt(\boldsymbol{\phi})\in\set C^{M\times K}$ is the basis matrix whose columns are the transmitter array response evaluated at the \glspl{AoD} in $\boldsymbol{\phi} = [\phi_1,\cdots,\phi_\K] \transp \in \set C^{K\times 1}$, i.e. 
%%%%%%%%%%%%%%%%%% Equation %%%%%%%%%%%%%%%%%% 
\begin{IEEEeqnarray}{lll} \label{Eq:CHt}
	\CHt(\boldsymbol{\phi})=\big[\mathbf{h}_t(\phi_1),\dots,\mathbf{h}_t(\phi_{K})\big].
\end{IEEEeqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Moreover, $\Cphi$ denotes the set of possible \glspl{AoD} and $\K$ is a design parameter and determines the number of \glspl{AoD} used for approximating the optimal precoder. Since in general the allowed feedback overhead is small, we choose $\K\ll LJ$. Therefore, the problem in \eqref{Eq:precoder} is equivalent to the sparse recovery problem in compressive sensing. \gls{OMP} is a widely-adopted algorithm, which can efficiently find the best $\K$ elements of basis matrix $\boldsymbol{\Psi}(\mathcal{C}_{\phi})\in\mathbb{C}^{M\times|\mathcal{C}_{\phi}|}$ to approximate $\mat{F}^{\mathrm{opt}}$~\cite{tropp2007signal}. Once $\boldsymbol{\phi}$ is derived, the optimization problem in \eqref{Eq:precoder} reduces to the well-known least square problem for $G$ whose closed-form solution is known. Algorithm~1 summarizes the proposed precoder design based on orthogonal matching pursuit.

\begin{algorithm}[t]
 	\caption{Feedback-Aware Precoding via Orthogonal Matching Pursuit}
 	\textbf{Require:} $\Fopt, \Cphi$
 	\begin{algorithmic}
 		\State 1: $\boldsymbol{\phi} = \text{Empty vector}$
 		\State 2: $\mat F_\text{res} = \Fopt$
 		\For{$i=1:\K$}
 		\State 4: $\mat Q = \CHt\hermis(\Cphi) \mat F_\text{res}$
 		\State 5: $\phi = {\mathrm{argmax}}_{l=1:|\Cphi|} (\mat Q \mat Q\hermis)_{l,l} $
 		\State 6: $\boldsymbol{\phi} = [\boldsymbol{\phi} , \phi]$
 		\State 7: $\mat G = \big(\CHt\hermis(\boldsymbol{\phi}) \CHt(\boldsymbol{\phi})\big)^{-1}  \CHt\hermis(\phi) \Fopt  $
 		\State 8: $\mat F_\text{res} = { {\Fopt-\CHt(\boldsymbol{\phi})\mat{G}} \over \frob{\Fopt-\CHt(\boldsymbol{\phi})\mat{G}} }$
 		\EndFor
 		\State 9: $\phiopt=\boldsymbol{\phi}$ and $\Gopt =  {\sqrt{S}\mat{G} \over \frob{\CHt(\boldsymbol{\phi})\mat{G}}}$
 		\State \textbf{Return} $\phiopt, \Gopt $
	\end{algorithmic} 
\end{algorithm}

Note that the transmitter only needs to know $\phiopt$ and $\Gopt$ to construct the precoder $\hat{\mat{F}}=\CHt(\phiopt)\Gopt$. Next, the transmitter can fully implement this precoder based on Lemma~1 for the hybrid MIMO architecture introduced in Section~\ref{sec:sysmod}.
The structure of precoder $\hat{\mathbf{F}}$ implies that the required feedback scales with $\K(1+S)$, which is not only independent of the number of transmit antennas $M$, but can also be controlled with the proposed design parameter $\K$.
Therefore, the solution of optimization problem \eqref{Eq:precoder} ensures that the set of the best $\K$ vectors for spanning the channel's row space and their corresponding combining matrix are fed back to the transmitter.
Consequently, the optimal precoder can be better approximated by choosing a larger $\K$ at the cost of increased feedback, while choosing a smaller $\K$ can lower the overhead when the feedback link bandwidth is limited.
We will study the effect of the parameter $K$ on the precoding performance in Section~\ref{sec:sim}.

%\vahid{---quantifying of the rate loss of $\hat{\mat{F}}$ by equation or somehow!}





\subsection{Extension to Multi-Beam Basis Elements}\label{subsec:non-modulo-one}
%The observation behind the proposed scheme in \eqref{Eq:precoder} %is that the optimal precoder can be written as the superposition of the transmitter array response vector at channel \glspl{AoD} with appropriate combining vectors. This
%implies the most immediate choice for the basis elements, i.e., columns of $\CHt(\boldsymbol \phi)$, be the transmitter array response vector, as defined in \eqref{Eq:CHt}.
The columns of the basis matrix $\CHt(\boldsymbol \phi)$ defined in \eqref{Eq:CHt}, are the transmitter array response vector at the angles in $\boldsymbol \phi$.
Recall that the angles in $\boldsymbol \phi$ are selected from the channel \gls{AoD} codebook $\Cphi$, where the transmitter sector is partitioned to sub-sectors by the codebook resolution and the middle angle of each sub-sector is naturally selected as the codebook elements.
Therefore, the higher the codebook resolution is, the better the beams of $\CHt(\Cphi)$ can approximate all possible \gls{AoD} realizations.
However, if the codebook resolution is forced to be low due to the constraint on the feedback link, the beams of $\CHt(\Cphi)$ cannot cover all the \gls{AoD} realizations in the transmitter beam sector and thus the performance of $\hat{\mat{F}}$ can be severely degraded.
Although this is a fundamental limitation of any precoder design scheme, it can be remedied for the proposed precoder.

Note that the MIMO architecture presented in Section~\ref{sec:sysmod} can implement any precoder matrix and hence the decomposition in \eqref{Eq:precoder} does not impose any implementation constraint on the basis matrix $\CHt(\boldsymbol{\phi})$.
Therefore, the structure of $\CHt(\boldsymbol \phi)$ only needs to be agreed by the transmitter and the receiver.
Motivated be the above, we propose to redefine $\CHt(\boldsymbol{\phi})$ in \eqref{Eq:precoder} and Algorithm~1 as
%%%%%%%%%%%%%%%%%% Equation %%%%%%%%%%%%%%%%%% 
\begin{IEEEeqnarray}{lll} \label{Eq:non_modulo1_array}
	\CHt(\boldsymbol{\phi})={1 \over \sqrt{\Gamma}} \Big[\sum_{\gamma=1}^{\Gamma}&\mathbf{h}_t\left(\phi_1-\frac{\Delta \phi}{2}+\frac{\gamma\Delta \phi}{\Gamma+1}\right),
	\dots, \nonumber \\ 
	&\sum_{\gamma=1}^{\Gamma}\mathbf{h}_t\left(\phi_K-\frac{\Delta \phi}{2}+\frac{\gamma\Delta \phi}{\Gamma+1}\right)  \Big],
\end{IEEEeqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\Delta\phi$ is the resolution of the \glspl{AoD} in $\Cphi$ and $\Gamma$ is a design parameter. This proposition implies that the beam candidate of each sub-sector is a superposition of $\Gamma$ beams of the angles from that sub-sector. By assuming $\Gamma=1$, the beam candidates become the array response vector at the middle angle of the corresponding sub-sector and thus \eqref{Eq:non_modulo1_array} is reduced to \eqref{Eq:CHt}.
Note that the proposition in \eqref{Eq:non_modulo1_array} does not impose any extra feedback overhead as $\Gamma$ is agreed by the transmitter and receiver. 

An example of the beam pattern resulting from the proposed approach is shown in Fig.~\ref{fig:beam}. These patterns are generated for $M=128$, $|\Cphi|=16$, and a sector covering $\phi\in[-\pi/6,\pi/6]$. In particular, in Fig.~\ref{fig:beam}, we show $g_k(\phi)$ versus $\phi$ where $g_k(\phi)$ is defined as 
%%%%%%%%%%%%%%%%%% Equation %%%%%%%%%%%%%%%%%% 
\begin{IEEEeqnarray}{lll}
	g_k(\phi) = \frac{|\mathbf{h}_t^*(\phi)\CHt(\phi_k)|^2}{\int_{\phi} |\mathbf{h}_t^*(\phi)\CHt(\phi_k)|^2\mathrm{d}\phi},
\end{IEEEeqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
characterizing the normalized power radiated in direction $\phi$ when $\CHt(\phi_k)$ is adopted as the RF beamformer.
As is shown in Fig.~\ref{fig:beam}, for $\Gamma= 1$, the power distribution across the sub-sector significantly varies with the angle and there are even several nulls within the sub-sector. This leads to a severe performance degradation when the \glspl{AoD} are actually at or close to these nulls. On the other hand, the power distribution across the sub-sector becomes more uniform when $\Gamma$ is increased. Nevertheless, by increasing $\Gamma$, the maximum achievable beamforming gain decreases and the interfering side lobes increase too. 
Therefore, $\Gamma$ provides a tradeoff for different \gls{AoD} codebook resolutions $|\Cphi|$. We will study the effect of this parameter on the precoder performance in Section~\ref{sec:sim}.

\begin{figure}[t]
	\centering
	%\includegraphics[width=\linewidth]{./fig/MultiBeam.eps}
	\input{./fig/multi_beam.tex}
	\caption{$g_k(\phi)$ vs. $\phi$ for $\phi_k=0$ and $\Gamma\in\{1,2,4\}$. The angles between the black vertical lines constitute the sub-sector that should be covered by the basis element $\mat{\Psi}(\phi_k)$.}
	\label{fig:beam}
\end{figure}





\subsection{Feedback Overhead Quantification}
In this subsection we quantify the feedback overhead of the proposed precoder. As explained, the receiver needs to feedback $\phiopt$ and $\Gopt$, which are realized by a codebook and individual quantized feedback, respectively.

\subsubsection{Overhead of $\phiopt$}
Recall that $\phiopt$ is the set of $\K$ \glspl{AoD} chosen from $\Cphi$ in \eqref{Eq:precoder}. Therefore, $\phiopt$ is naturally encoded by quantization of the \glspl{AoD} in $\Cphi$. Assuming a uniform quantization, each angle in the codebook is encoded by $\mathrm{log_2}|\Cphi|$ bits and thus the feedback overhead for $\phiopt$ is $\K \,\mathrm{log_2}|\Cphi|$ bits.

\subsubsection{Overhead of $\Gopt$}
The overhead required to feed back $\Gopt$ to the transmitter depends on the structure of $\Gopt$. We discuss three cases.
For the most general case when $\Gopt$ is an arbitrary complex matrix, the feedback overhead scales with $\K S$. Let, $\mathcal{C}_{\mathbf{G}}$ denotes the set of quantized complex number. Thereby, the feedback overhead is $\K S\,\mathrm{log_2}|\mathcal{C}_{\mathbf{G}}|$ bits. Nevertheless, $\Gopt$ can be designed to have a specific structure that allows for a less overhead. For instance, matrix $\Gopt$ can be made unitary, i.e., $(\Gopt)\hermis\Gopt=\mathbf{I}_{S}$.\footnote{Having a unitary $\mathbf{G}$ implies that no power allocation across different data streams is applied, i.e., $\alpha_1=\alpha_2=\dots=\alpha_S$. In addition, Step 7 of the proposed Algorithm~1 has to be revised to enforce that the columns of $\mathbf{G}$ are orthogonal, see~\cite{el2014spatially} for further discussion. }
In this case, efficient codebooks can be designed for $\Gopt$ using Lloyd's algorithm and the chordal distance as a distance measure, see \cite{el2014spatially} and the references therein for a more detailed discussion. Finally, $\Gopt$ can be designed such that in each column, it has only one non-zero element equal to one. In other words, each \gls{AoD} is assigned only to one data stream. For this scheme, the feedback overhead is upper bounded by %$\K \,\mathrm{log_2}S$ bits.
$K\log_2(S)+K\log_2|\mathcal{C}_{\mathbf{G}}|$, where $K\log_2(S)$ and $K\log_2|\mathcal{C}_{\mathbf{G}}|$ quantify the required feedback for determining the positions of the non-zero elements in the columns of $\mathbf{G}$ and their values, respectively.
The following lemma formally states that the aforementioned strategy yields the optimal unconstrained precoder as $M\to\infty$.

\begin{lem}
Asymptotically as $M\to\infty$, $\Gopt$ as the solution of (\ref{Eq:precoder}) has the form $\Gopt\to[\mathbf{A},\mathbf{0}_{S\times (\K-S)}]\transp$ when $\K \geq S$ and $\mathbf{A}$ is a diagonal matrix with $\alpha_1,\dots,\alpha_S$ as its diagonal elements.
\end{lem}
\begin{IEEEproof}
As $M\to\infty$, the columns of matrix $\mat{H}_t(\boldsymbol{\phi})$ become orthogonal~\cite{el2012capacity}. Thereby, the columns of the optimal matrix $\Fopt$ become identical to the scaled version of the first $S$ columns of $\mat{H}_t(\boldsymbol{\phi})$, where the scaling factors are the power allocation variables. Therefore, assuming $\K \geq S$, matrix $\Fopt$ can be fully reconstructed from (\ref{Eq:precoder}) by choosing $\Gopt=[\mathbf{A},\mathbf{0}_{S\times (\K -S)}]\transp$. This completes the proof.
\end{IEEEproof}

The above lemma states that asymptotically as $M\to\infty$, simple beam steering along the $S$ dominant \gls{AoA} is optimal. Therefore, one can choose $\K=S$. Moreover, if the sum rate is the performance metric, it does not matter which stream is assigned to which \gls{AoA} and since each stream should be assigned to one \gls{AoA}, matrix $\Gopt$ constructed by any permutation of the columns of identity matrix $\mathbf{A}$ is optimal.
Note that in finite regime of $M$, the above results is not valid; however, it provides a design intuition for a suboptimal precoder with limited feedback requirement. 

\subsubsection{Total feedback overhead}
We summarize the total required feedback of the proposed precoder in the following lemma that states a bound on the overhead requirement for the non-asymptotic scenario, i.e., finite $M$.
\begin{lem}
	To approach the performance of the fully-digital system, the feedback requirement of the proposed precoding scheme is on the order of $LJ(\mathrm{log_2}|\Cphi|+S\mathrm{log_2}|\mathcal{C}_{\mathbf{G}}|)$ bits assuming that $|\Cphi|$ and $|\mathcal{C}_{\mathbf{G}}|$ are sufficiently large.	
\end{lem}
\begin{IEEEproof}
	For the non-asymptotic regime of $M$, the columns of the optimal unitary matrix $\Fopt$ may depend on the array response of all existing \glspl{AoA}. Therefore, we choose $\K=LJ$. Subsequently, $\hat{\mathbf{F}}$ approaches $\Fopt$ assuming that $|\Cphi|$ and $|\mathcal{C}_{\mathbf{G}}|$ are sufficiently large. This leads to an overhead requirement of $LJ(\mathrm{log_2}|\Cphi|+S\mathrm{log_2}|\mathcal{C}_{\mathbf{G}}|)$ bits, which concludes the proof.
\end{IEEEproof}

The above lemma states that as long as the \gls{mmWave} channel contains limited scattering, i.e., $LJ\ll M$, the proposed scheme can effectively approach the performance of a fully-digital system with a limited feedback requirement that linearly scales with $LJ$.   

%\vahid{--- Rx Complexity analysis}
